Randomize the Future: Asymptotically Optimal Locally Private Frequency Estimation Protocol for Longitudinal Data

Longitudinal data tracking under Local Differential Privacy (LDP) is a challenging task. Baseline solutions that repeatedly invoke a protocol designed for one-time computation lead to linear decay in the privacy or utility guarantee with respect to the number of computations. To avoid this, the recent approach of Erlingsson et al. (2020) exploits the potential sparsity of user data that changes only infrequently. Their protocol targets the fundamental problem of frequency estimation protocol for longitudinal binary data, with $\ell_\infty$ error of $O ( (1 / \epsilon) \cdot (\log d)^{3 / 2} \cdot k \cdot \sqrt{ n \cdot \log ( d / \beta ) } )$, where $\epsilon$ is the privacy budget, $d$ is the number of time periods, $k$ is the maximum number of changes of user data, and $\beta$ is the failure probability. Notably, the error bound scales polylogarithmically with $d$, but linearly with $k$. In this paper, we break through the linear dependence on $k$ in the estimation error. Our new protocol has error $O ( (1 / \epsilon) \cdot (\log d) \cdot \sqrt{ k \cdot n \cdot \log ( d / \beta ) } )$, matching the lower bound up to a logarithmic factor. The protocol is an online one, that outputs an estimate at each time period. The key breakthrough is a new randomizer for sequential data, FutureRand, with two key features. The first is a composition strategy that correlates the noise across the non-zero elements of the sequence. The second is a pre-computation technique which, by exploiting the symmetry of input space, enables the randomizer to output the results on the fly, without knowing future inputs. Our protocol closes the error gap between existing online and offline algorithms.

==> improved-soln.tex <==
\section{\algoImproved} \label{sec:improved private algorithm}

The result we obtain in the previous section has a factor $\frac{ e^{\eps / k} + 1 }{ e^{\eps / k} - 1} \in O(k / \eps)$ in the error bound, as Algorithm~\ref{algo:Basic Client} invokes the randomizer~$\cM$ with privacy budget $\eps / k$ each time.
For each $h \in \IntSet{0}{\log d}$, there can be at most $k$ non-zero partial sums associated with dyadic intervals with order~$h$, hence the final algorithm is $\eps$ differentially private.
It motivates to allocate less privacy budget to reduce the error bound.
This is possible if we treat the non-zero elements as a whole.

\begin{theorem} \label{theorem: property of improved private algorithm}
    Assuming that $\eps \le 1$, $k \ge 126$ and $\sqrt{n} \ge  (1 / \eps) \cdot \sqrt{k \cdot \paren{ \ln k + \ln (1 / \eps) } } \cdot (\log d) \cdot \sqrt{ \ln \paren{d / \beta} } $, there is an $\eps$- local differentially private protocol, such that with probability at least $1 - \beta$, its estimations $\EstPorpulationSum{t}$ of $\PorpulationSum{t}$ satisfies
    $$
        \max_{t \in [d] } \card{ \EstPorpulationSum{t} - \PorpulationSum{t} } 
        \in  
        O \paren{ \frac{ \sqrt{k \cdot \paren{ \ln k + \ln (1 / \eps) } } } {\eps} \cdot (\log d) \cdot \sqrt{  n  \cdot \ln \frac{d}{\beta} }  }.
    $$
\end{theorem}

\subsection{Composed Randomizer}

Our algorithm invokes the advanced composition algorithm proposed by~\citeauthor{BNS19}~\citep{BNS19} as a subroutine, described in Algorithm~\ref{algo:Approximate Composed Algorithm}.  
The original algorithm accepts inputs that are sequences consisting of $0$ and $1$, and outputs a sequences of $0$ and $1$.
We observe that this is not essential, and the algorithm can be converted to work with arbitrary binary inputs.  
Therefore, the algorithm we present here has  input sequences that contain $-1$ and $1$, and outputs a sequences of $-1$ and $1$. 

Suppose that user $u \in [n]$ has a sequence $B_u \in \set{-1, 1}^k$. 
If we independently apply $\cM{}$ to each coordinate of $B_u$ with some privacy parameter~$\tildeeps$, in expectation, we changes~$k / (e^{\tildeeps} + 1)$ coordinates of $B_u$. 
Denote $p \doteq 1 / ( e^{ \tildeeps } + 1)$ and 
\begin{equation}
      \pavg \doteq \paren{ p }^{  k p  } \paren{ 1 - p }^{ k \paren{ 1 - p } }.
\end{equation}
For each~$W \in \{ -1, 1 \}^k$ such that $\norm{ B_u - W }_0 = kp$ (where~$\norm{ \cdot }_0$ is the $\ell_0$ norm, and therefore~$\norm{ B_u - W }_0$ is the Hamming distance between~$B_u$ and~$W$), it holds that 
$$
    \P{ \paren{ \cM ( B_u [1], \tildeeps), \ldots, \cM ( B_u [k] , \tildeeps) } = W } = \pavg.
$$
Intuitively, if for each~$W \in \{ -1, 1 \}^k$, it holds that 
\begin{equation} \label{equa: key for private}
    \P{ \paren{ \cM ( B_u [1], \tildeeps), \ldots, \cM ( B_u [k] , \tildeeps) } = W }
    \approx \pavg,\,
\end{equation}
then it is hard to to infer the value of $B_u$ based on~$W$, making the algorithm private.
However, Equation~(\ref{equa: key for private}) holds only for those~$W$ whose~$\norm{ B_u - W }_0$ are close to~$kp$.

Motivated by this observation, Algorithm~\ref{algo:Approximate Composed Algorithm} treats those~$W$ whose~$\ell_0$ distance to~$B_u$ are close to~$kp$ and the ones whose~$\ell_0$ distance to~$B_u$ are far from~$kp$ differently. 
For some~$\lambda \in (0, 1)$ to be determined later, define
\begin{definition}[Annulus] Given $B_u \in \set{-1, 1}^k$, denote
$$
    \Annulus{B_u}
    \doteq \set{ W \in \set{-1, 1}^k : \card{ \norm{ B_u - W }_0 - kp } \le \sqrt{ \frac{ k } { 2 } \cdot  \ln \frac{ 2 } { \lambda }  } }
$$
\end{definition}
Algorithm~\ref{algo:Approximate Composed Algorithm} regards those~$W \in \Annulus{B_u}$ with~$\norm{ B_u - W }_0$ close to~$kp$. 
If~$\paren{ M(B_u [1]), \ldots, M(B_u [k]) } \in \Annulus{B_u}$, then the algorithm outputs it directly. 
Otherwise, it outputs an element from~$\set{-1, 1}^k \setminus \Annulus{B_u}$ uniformly at random. 
This enforces those~$W$ whose $\ell_0$ distances are far from $kp$ to have the same output probability. 







\begin{algorithm}[!ht]
    \caption{Approximate Composed Algorithm $\tilde \cM{} (B_u, \tildeeps)$}
    \label{algo:Approximate Composed Algorithm}
        \begin{algorithmic}[1]
            \Require Vector $B_u \in \set{-1, 1}^k$; Privacy parameter $\tildeeps$.
            \State Sample $W \leftarrow ( \cM ( B_u [1], \tildeeps), \ldots, \cM ( B_u [k] , \tildeeps) )$.
            \label{algo line: 1 algo:Approximate Composed Algorithm}
            \If{ $W \notin \Annulus{B_u}$ }
                \State $W \leftarrow$ uniform random sample from $\set{-1, 1}^k \setminus \Annulus{B_u}$
                \label{algo line: 3 algo:Approximate Composed Algorithm}
            \EndIf
            \State {\bf return} $W_u \leftarrow W$
        \end{algorithmic}
\end{algorithm}

\noindent The property of Algorithm~\ref{algo:Approximate Composed Algorithm} is summarized as follows. 

\begin{fact}[Algorithm~\ref{algo:Approximate Composed Algorithm}~\citep{BNS19}] \label{fact: probability of elements outside typicall set}
    Suppose that 
    \begin{equation} \label{ineq: lambda tilde eps and k}
        0 < \lambda < \paren{ \tildeeps \sqrt{k} / \paren{2 (k + 1)}  }^{2 / 3}\,,
    \end{equation}
    and that
    \begin{equation} \label{eq: eps and tilde eps}
        \eps = 6 \tildeeps \sqrt{k \ln (1 / \lambda) } \le 1.
    \end{equation}
    The algorithm $\tilde{\cM} : \set{-1, 1 }^k \rightarrow \set{-1, 1}^k$ is $\eps$ differentially private.
    In particular, for each~$W  \in \Annulus{B_u}$,  
    $$
        \P{ \tilde{\cM} (B_u, \tilde{ \eps } ) = W  } \in 
        \left[ 
            e^{-\tilde{ \eps } \sqrt{ (k / 2) \ln (1 / \lambda) } }, e^{ \tilde{ \eps } \sqrt{ (k / 2) \ln (1 / \lambda) } } 
        \right] \cdot 
        \pavg,\,
    $$
    and for each $W  \in \set{-1, 1}^k \setminus \Annulus{B_u}$, 
    $$
        \P{ \tilde{\cM} (B_u, \tilde{ \eps } ) = W  } \in \left[ 
            e^{-3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } }, e^{ 3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } } 
        \right] \cdot 
        \pavg.
    $$
\end{fact}

We can derived the following constraint between~$\lambda$, $\eps$ and~$k$. 

\begin{theorem}
    If $\lambda$ satisfies Inequality~(\ref{ineq: lambda tilde eps and k}) and Equality~(\ref{eq: eps and tilde eps}), then 
    $\ln (1 / \lambda) \in \Omega ( \ln ( k / \eps) )$.
\end{theorem}
\begin{proof}
    Substituting $\tildeeps = \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) }}$ into Inequality~(\ref{ineq: lambda tilde eps and k}), we get 
    \begin{align*}
        \lambda^{3 / 2} 
            < \frac{\eps \sqrt{k} }{ 6 \sqrt{k \ln (1 / \lambda) } \cdot 2(k + 1)} 
        \implies
            \frac{3}{2} \ln \lambda + \frac{1}{2} \ln \ln \frac{1}{\lambda} < \ln \frac{ \eps }{ 12 (k + 1) }.
    \end{align*}
    Therefore, $\ln (1 / \lambda) \in \Omega ( \ln ( k / \eps) )$.
\end{proof}


\subsection{Client Side}

The users can not apply $\tilde{\cM}$ to randomize the non-zero partial sums directly for two reasons: 1) the number of non-zero partial sums of dyadic intervals with the chosen order does not equal exactly to $k$; 2) the users need to know all non-zero partial sums before invoking $\tilde{\cM}$, which prevents the server from outputting $\EstPorpulationSum{t}$ at time $t$, for $t < d$.

Instead, each user~$u \in [n]$ invokes $\tilde{\cM}(1^k, \tildeeps)$, and regards the outputs as random bits, where $1^k$ is the vector the consists of $k$ ones and $\tildeeps$ is the privacy budget whose value will be discussed later.
Denote the output as $W_u \in \set{-1, 1}^k$.
For each $j \in [k]$, the user~$u$ perturbs the $j^{ (th) }$ non-zero partial sum (if exits) by multiplying it by $W_u [j]$.
If $W_u [j] = 1$, this partial sum is reported faithfully to the server; otherwise, the sign of it is reversed.
The detailed algorithm is described in Algorithm~\ref{algo:Client}.

\begin{algorithm}[!ht]
    \caption{Client $\algoClient{}$}
    \label{algo:Client}
        \begin{algorithmic}[1]
            \Require Data $X_u \in \set{-1, 0,  1}^d$; Privacy parameter $\epsilon$.
            \State Sample an~$h_u \in \IntSet{0}{\log d}$ uniformly at random.     
            \State  
            $\lambda \leftarrow \frac{\eps}{12 (k + 1) \sqrt{ 1 + \ln (1 / \eps) }}$,\,
            $\tildeeps \leftarrow \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) }} $
            \State $L \leftarrow d / 2^{h_u}$;\,
            $\pmbomega{}_u \leftarrow \set{0}^{ L }$;\, 
            $W_u \leftarrow \tilde{\cM}( 1^k, \tildeeps{})$;\, 
            $j \leftarrow 0$;
            \For{$\ell \in [L]$ } 
                \If{$\partialsum{u}{ \dyadicInterval{ h_u }{ \ell } } \neq 0$}
                    \State $j \leftarrow j + 1$.
                    \State $\pmbomega_u [ \ell ] \leftarrow \partialsum{u}{ \dyadicInterval{ h_u }{ \ell } } \cdot W_u [j]$.
                \Else
                    \State $\pmbomega_u[ \ell ] \leftarrow$ $-1$ or $+1$ uniformly at random.
                \EndIf
            \EndFor
            \State {\bf return} $\Big( h_u, \pmbomega{}_u \Big)$.
        \end{algorithmic}
\end{algorithm}

\noindent {\bf Privacy Guarantee.} 
We discuss the privacy guarantee offered by Algorithm~\ref{algo:Client}. 

\begin{lemma} \label{lemma: output probability range of client}
    For each user data~$\UsrDerivative{u} \in \set{-1, 0, 1}^d$, each~$h \in \IntSet{0}{\log d}$, and each~$\pmbomega \in \set{-1, 1}^{ \card{\dyadicIntervalSet{h} } }$,
    \begin{equation*} \label{ineq: client output prob}
        \P{ \algoClient{}( X_u, \eps{}  ) = (h, \pmbomega{}) } 
        \in \frac{ \pavg }{ 1 + \log d } 
        \cdot 2^{- ( \card{\dyadicIntervalSet{h} } - k )} 
        \cdot \left[ 
               e^{ - \eps / 2}, e^{ \eps / 2}
        \right].
    \end{equation*}
\end{lemma} 

\noindent We defer the proof of the lemma to the end of this subsection.
By similar proof as the one of Theorem~\ref{theorem: client basic is private}, we immediately obtain the following the theorem. 

\begin{theorem} 
    Algorithm~\ref{algo:Client} is $\eps$ differentially-private.
\end{theorem}

\begin{proof}[{Proof of Lemma~\ref{lemma: output probability range of client}}]
    For a fixed $\UsrDerivative{u}$.
    For each~$h \in \IntSet{0}{\log d}$, $$
        \Pr[ h_u = h ] = 1 / (1 + \log d).
    $$
    Now, suppose~$h_u = h$. 
    Denote~$L = \card{\dyadicIntervalSet{ h_u } }$. 
    Define the set of dyadic intervals with order~$h_u$ whose associated partial sums are not zero as
    $$
        \supp{ h_u } \doteq \set{ \ell \in   [L] : \partialsum{u}{ \dyadicInterval{h_u}{\ell} } \neq 0 }.
    $$
    According to Observation~\ref{observation: basic partial sum properties}, $\card{ \supp{ h_u } } \le k$.
    Consider the following two events: 
    \begin{enumerate}
        \item~$E_1:$ $\forall \ell \notin \supp{ h_u }$, $\pmbomega{}_u [ \ell ] = \pmbomega{}[ \ell ]$.
        \item~$E_2:$ $\forall \ell \in \supp{ h_u }$, $\pmbomega{}_u [ \ell ] = \pmbomega{}[ \ell ]$.
    \end{enumerate}
    First, for each $\ell \notin \supp{ h_u }$, we have that $\partialsum{u}{ \dyadicInterval{u}{\ell} } = 0$, and $\pmbomega{}_u [ \ell ]$ equals $-1$ or $+1$ independently uniformly at random. 
    Therefore, 
    $$
        \P{ E_1 } = \prod_{ \ell \notin \supp{ h_u } } \P { \pmbomega{}_u [ \ell ] = \pmbomega{}[ \ell ] } = 1 / 2^{ L - \card{ \supp{ h_u } } }. 
    $$
    
    \noindent Second, consider~$E_2$.
    Assume the indexes in $\supp{ h_u }$ are
    $$
        \ell_1 < \ell_2 < \ldots < \ell_{ \card{ \supp{h_u} } }. 
    $$
    For each $j \in [\card{ \supp{h_u} }]$, since $\pmbomega{}_u [ \ell_j ] = \partialsum{u}{ \dyadicInterval{ h_u }{ \ell_j } } \cdot W_u [j]$, it holds that 
    $\pmbomega{}_u [ \ell_j ] = \pmbomega{}[ \ell_j ]$ if only 
    $\partialsum{u}{ \dyadicInterval{ h_u }{ \ell_j } } \cdot W_u [j] = \pmbomega{}[ \ell_j ]$, i.e., 
    \begin{equation} \label{equa: requirement of W}
        W_u [j] = 
        \frac{ \pmbomega{}[ \ell_j ] }
        {
            \partialsum{u}{ \dyadicInterval{ h_u }{ \ell_j } }
        }.
    \end{equation}
    According to Algorithm~\ref{algo:Client}, $W_u$ is the output vector of~$\tilde{\cM}( 1^k, \tildeeps{})$.
    Denote the set of possible outputs for which Equation~(\ref{equa: requirement of W}) is satisfied:
    $$
        \targetOutputs 
        \doteq 
        \set{ 
            W \in \set{-1, 1}^k : 
            \forall j \in [\card{ \supp{h_u} }], 
            W[j] = 
            \frac{ \pmbomega{}[ \ell_j ] }
            {
                \partialsum{u}{ \dyadicInterval{ h_u }{ \ell_j } }
            }
        }.
    $$
    Via Fact~\ref{fact: probability of elements outside typicall set}, it always holds that for each $W \in \targetOutputs$, 
    $$
        \P{ \tilde{\cM} (B_u, \tilde{ \eps } ) = W  } \in \left[ 
            e^{-3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } }, e^{ 3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } } 
        \right] \cdot 
        \pavg.
    $$
    Summing over the $2^{ k - \card{ \supp{h_u} } }$ possible sequences in~$\targetOutputs$, we see that $\P{ E_2 } = \P{ \tilde{\cM} (B_u, \tilde{ \eps } ) \in \targetOutputs}$ is bounded by 
    $$
        2^{k - \card{ \supp{ h_u } } } \cdot 
        \left[ 
                e^{-3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } }, e^{ 3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } } 
        \right] \cdot 
        \pavg.
    $$
    Therefore, $\P{ \algoClient{}( X_u, \eps{}  ) = (h, \pmbomega{}) }$ is bound by 
    $$
       \frac{ 1 }{ 1 + \log d } \cdot 2^{- ( L - k )} \cdot 
        \left[ 
                e^{-3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } }, e^{ 3 \tilde{ \eps } \sqrt{ k \ln (1 / \lambda) } } 
        \right] \cdot 
        \pavg.
    $$
    Substituting again $3 \tildeeps \sqrt{k \ln (1 / \lambda) }$ with $\eps / 2$ proves Inequality~(\ref{ineq: client output prob}). 
\end{proof}






\subsection{Server Side Algorithm}

{\bf Report Processing.}
The report processing procedure is almost the same as Algorithm~\ref{algo:Basic Server}, except that it replaces the scaling factor~$\cSvrBasic$ with a new one~$\cSvr$, which is the reciprocal of the $\P{ W_u [1] = 1 } - \P{ W_u [1] = -1 }$: 
$$
    \cSvr = 1 / \paren{ \P{ W_u [1] = 1 } - \P{ W_u [1] = -1 } }.  
$$
Since $W_u \leftarrow \tilde{\cM}( 1^k, \tildeeps{})$, by symmetry, it holds that 
$$
    1 / \cSvr = { \P{ W_u [j] = 1 } - \P{ W_u [j] = -1 } },\, \forall j \in [k]. 
$$
The~$\cSvr$ can be computed as follows. 
Let 
\begin{align}
    \Lb \doteq kp - \sqrt{ (k / 2) \ln (2 / \lambda) },\,
    \Ub \doteq kp + \sqrt{ (k / 2) \ln (2 / \lambda) }.
\end{align}
Observe that for each $W_u \notin \Annulus{1^k}$, $\P{ \tilde{\cM} (1^k , \tildeeps) = W_u }$ equals 
\begin{equation}
    \PrOut 
    \doteq 
    \frac{ 
        \sum_{ i = 0}^{ \Lb - 1} \binom{k}{i} p^i (1 - p)^{k - i} + \sum_{ i = \Ub + 1}^{ k } \binom{k}{i} p^i (1 - p)^{k - i} 
    }
    {
        \sum_{ i = 0}^{ \Lb - 1} \binom{k}{i} + \sum_{ i = \Ub + 1}^{ k } \binom{k}{i}
    }.
\end{equation}
Let $\overline{ \IntSet{\Lb}{\Ub} } \doteq \IntSet{0}{k} \setminus \IntSet{\Lb}{\Ub}$. 
Then $\P{ W_u[1] = 1 }$ equals
\begin{equation*}
    \sum_{ i = \Lb }^{ \Ub} p^i (1 - p)^{k - i}  \binom{k}{i} \paren{1 - \frac{i}{k} } 
        + \sum_{ i \in \overline{ \IntSet{\Lb}{\Ub} } } \PrOut \binom{k}{i} \paren{1 - \frac{i}{k} },
\end{equation*}
and~$\P{ W_u[1] = -1 }$ is given by 
\begin{equation*}
    \small
    \sum_{ i = \Lb }^{ \Ub} p^i (1 - p)^{k - i}  \binom{k}{i} \frac{i}{k}
    + \sum_{ i \in \overline{ \IntSet{\Lb}{\Ub} } } \PrOut \binom{k}{i} \frac{i}{k}.
\end{equation*}
It follows that 
\begin{equation} \small
    \frac{1}{\cSvr} = \sum_{ i = \Lb }^{ \Ub} p^i (1 - p)^{k - i}  \binom{k}{i} \paren{1 - \frac{2i}{k} } 
    + \sum_{ i \in \overline{ \IntSet{\Lb}{\Ub} } } \PrOut \binom{k}{i} \paren{1 - \frac{2i}{k} }.
\end{equation}

\noindent {\bf Query.} 
The query algorithm is exactly the same as Algorithm~\ref{algo:Basic Query}.

\noindent {\bf Determining~$\tildeeps$ and~$\lambda$.} 
Observe that~$1 / \cSvr$ is the gap between the probabilities that some coordinate is preserved and that such coordinate is reversed. 
The smaller this gap is, the more difficult for the server to recover the true coordinate and the larger the estimation error. 
The following lemma states that, if~$\lambda$ is not too large, then $1 / \cSvr$ is lower bounded. 

\begin{lemma} \label{lemma: upper on Gamma}
    If 
    \begin{equation} \label{ineq: lambda and tilde eps}
        \lambda \le \paren{1 / 4} \cdot \paren{ e^{ \tildeeps} - 1 } / \paren{ e^{ \tildeeps} + 1 }, 
    \end{equation}
    then 
    \begin{equation}
        1 / \cSvr \ge \paren{1 / 2} \cdot \paren{ e^{ \tildeeps} - 1 } / \paren{ e^{ \tildeeps} + 1 }.
    \end{equation}
\end{lemma}

\begin{theorem} \label{theorem: setting of epsilon lambda}
    Assuming that $k \ge 126$. 
    If we set 
    \begin{equation} \label{equa: value of lambda}
        \lambda \doteq \frac{\eps}{12 (k + 1) \sqrt{ 1 + \ln (1 / \eps) }}   
    \end{equation}
    and 
    \begin{equation} \label{equa: value of tildeeps}
        \tildeeps 
        \doteq \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) }} 
        = \frac{\eps}{6 \sqrt{k \ln \paren{ 12 (k + 1) \sqrt{ 1 + \ln (1 / \eps) } / \eps }  } },
    \end{equation}
    then Inequalities~(\ref{ineq: lambda tilde eps and k},~\ref{ineq: lambda and tilde eps}), and  Equation~(\ref{eq: eps and tilde eps}) hold.
\end{theorem}



\begin{proof}[Proof of Lemma~\ref{lemma: upper on Gamma}.]
    Since $W_u = \tilde{M} (1^k, \tildeeps)$, if $W_u[1] = 1$, either of the following events happens
    \begin{enumerate}
        \item $M(1, \tildeeps) = 1$ (line~\ref{algo line: 1 algo:Approximate Composed Algorithm} of Algorithm~\ref{algo:Approximate Composed Algorithm}). 
        \item $W$ is a random sample from $\set{-1, 1}^k \setminus  \Annulus{1^k}$ (line~\ref{algo line: 3 algo:Approximate Composed Algorithm} of Algorithm~\ref{algo:Approximate Composed Algorithm}).
    \end{enumerate}
    The former happens with probability $e^{ \tildeeps} / ( e^{ \tildeeps} + 1)$ and the later happens with probability at most $\lambda$ (by Hoeffding's inequality). 
    Via union bound, we have 
    $$
        \P{ W_u [1] = 1 } \le e^{ \tildeeps} / ( e^{ \tildeeps} + 1) + \lambda. 
    $$
    Similarly, we can derive 
    $$
        \P{ W_u [1] = -1 } \le 1 / ( e^{ \tildeeps} + 1) + \lambda. 
    $$
    Therefore,
    \begin{align*}
        1 / \cSvr 
            &=\P{ W_u [1] = 1 } - \P{ W_u [1] = -1 } \\
            &= 1 - \P{ W_u [1] = -1 } - \P{ W_u [1] = -1 } \\
            &= 1 - 2 \P{ W_u [1] = -1 } \\
            &\ge 1 - 2 / \paren{ e^{ \tildeeps} + 1 } - 2 \cdot \lambda \\
            &= \paren{ e^{ \tildeeps} - 1 } / \paren{ e^{ \tildeeps} + 1 } - 2 \cdot \lambda. 
    \end{align*}
    Combing with that $\lambda \le (1 / 4) \cdot ( e^{\tildeeps} - 1 ) / ( e^{\tildeeps } + 1 )$ finishes the proof. 
\end{proof}

\begin{proof}[Proof of Theorem~\ref{theorem: setting of epsilon lambda}.]
    As we set~$\lambda$ according to Equation~(\ref{equa: value of lambda}), 
    Equation~(\ref{eq: eps and tilde eps}) holds trivially. 
    It is left to verify Inequalities~(\ref{ineq: lambda tilde eps and k}) and~(\ref{ineq: lambda and tilde eps}).  
    
    \noindent {\bf Inequalities~(\ref{ineq: lambda tilde eps and k}):}
    Substituting~$\tildeeps = \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) } }$ (Equation~(\ref{equa: value of tildeeps})), Inequalities~(\ref{ineq: lambda tilde eps and k}) reduces to 
    \begin{align*}
        0 < \lambda 
        \le \paren{ \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) } }  \frac{ \sqrt{k} }{ \paren{2 (k + 1)} } }^{2 / 3} 
        = \paren{ \frac{\eps}{12 (k + 1) \sqrt{ \ln (1 / \lambda) }} }^{2 / 3}. 
    \end{align*}
    It is left to verify this inequality. 
    Observe that Equation~(\ref{equa: value of lambda}) implies that $\lambda \le \eps / \paren{ 12 \paren{ k + 1}}$. 
    Combing with the fact that $\ln (1 / \lambda) \le 1 / \lambda$, 
    $$
        \paren{ \frac{\eps}{12 (k + 1) \sqrt{ \ln (1 / \lambda) }} }^{2 / 3}
        \ge 
        \paren{ \frac{ \lambda }{ \sqrt{ 1 / \lambda }} }^{2 / 3} = \lambda. 
    $$
    
    \noindent {\bf Inequalities~(\ref{ineq: lambda and tilde eps}):}
    Note that 
    \begin{align*} \small
        \frac{1}{4} \cdot \frac{ e^{\tildeeps} - 1 }{ e^{\tildeeps } + 1 }
        \ge \frac{1}{4 ( e^{\tildeeps } + 1 ) } \tildeeps
        \ge \frac{1}{4 ( e^{1 / 12} + 1 ) } \tildeeps,
    \end{align*}
    where the first inequality follows from that $e^x - 1 \ge x$ for all $x \in \R$, and the last inequality from that $\eps < 1$ and $\tildeeps = \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) } } \le \frac{1}{ 6 \sqrt{k} } \le \frac{1}{12}$, since $\ln \paren{1 / \lambda} > 1$ and as we assume that~$k > 126$.  
    
    Inequality~(\ref{ineq: lambda and tilde eps}) holds, if $\lambda \le \frac{1}{4 (e^{1 / 12} + 1) } \tildeeps$. 
    Substituting~$\tildeeps = \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) } }$ (Equation~(\ref{equa: value of tildeeps})), we need to verify
    \begin{align*}
        \lambda \le \frac{1}{4 (e^{1 / 12} + 1) } \frac{\eps}{6 \sqrt{k \ln (1 / \lambda) } }. 
    \end{align*}
    
    Via Equation~(\ref{equa: value of lambda}), we see that $\lambda / \eps = 1 / \paren{ 12 \paren{k + 1} \sqrt{1 + \ln \paren{1 / \eps}} }$. 
    It reduces to prove that 
    \begin{align*}
        &\frac{1}{ 12 \paren{k + 1} \sqrt{1 + \ln \paren{1 / \eps}} } 
        \le 
        \frac{1}{4 (e^{1 / 12} + 1) } \frac{1}{6 \sqrt{k \ln (1 / \lambda) } }.
    \end{align*}
    Equivalently, 
    \begin{align} \label{ineq: derived k lambda eps}
        \sqrt{ k \ln (1 / \lambda) } 
        \le \frac{ \paren{k + 1} \sqrt{1 + \ln \paren{1 / \eps}} }{ 2 (e^{1 / 12} + 1) }.
    \end{align}
    Substituting again~$\lambda / \eps = 1 / \paren{ 12 \paren{k + 1} \sqrt{1 + \ln \paren{1 / \eps}} }$, 
    \begin{align*}
        \ln \paren{1 / \lambda} 
            &= \ln \paren{ 12 (k + 1) \sqrt{ 1 + \ln (1 / \eps) } / \eps } \\
            &= \ln \paren{ 12 (k + 1)} + (1 / 2) \ln  \paren{ 1 + \ln (1 / \eps) }  + \ln \paren{1 /  \eps } \\
            &\le \ln \paren{ 12 (k + 1)} + (1 / 2) \ln \paren{1 /  \eps } + \ln \paren{1 /  \eps } \\
            &=  \ln \paren{ 12 (k + 1)} + (3 / 2) \ln \paren{1 /  \eps },  
    \end{align*}
    where the inequality holds since $\ln (1 + x) \le x$ for $x \ge 0$ and that $\ln (1 / \eps) > 0$ by~$\eps < 1$. 
    Inequality~(\ref{ineq: derived k lambda eps}) holds if 
    \begin{align*}
        k \paren{ \ln \paren{ 12 (k + 1)} + (3 / 2) \ln \paren{1 /  \eps } }
        &\le \paren{ \frac{ k + 1}{ 2 (e^{1 / 12} + 1) } }^2  \paren{ 1 + \ln (1 / \eps ) } 
    \end{align*}
    
    \noindent It can be verified that when $k \ge 126$, it holds
    $$
        \paren{ \frac{ k + 1}{ 2 (e^{1 / 12} + 1) } }^2 \ge k \ln (12 (k + 1) ),\,
        \paren{ \frac{ k + 1}{ 2 (e^{1 / 12} + 1) } }^2 \ge k (3 / 2),
    $$
    which finishes the proof.
  
\end{proof}








\noindent {\bf Utility Guarantee.}  
The following theorems investigate the qualities of the estimations $\EstPorpulationSum{t}$.

\begin{theorem} \label{theorem: unbiased estimator for private algorithm}
    $\forall t \in [d]$, $\EstPorpulationSum{t}$ is an unbiased estimator of $\PorpulationSum{t}$.
\end{theorem}


\begin{theorem} \label{theorem: error of single estimator for private algorithm}
    For each $t \in [d]$, assuming that $\eps \in O(k)$ and that $\sqrt{n} \ge \frac{k}{\eps} \cdot (\log d) \cdot \sqrt{ \ln \frac{1}{\beta} }$, with probability at least $1 - \beta$, we have
    $$
        | \EstPorpulationSum{t} - \PorpulationSum{t} | \in  O \paren{ \frac{k}{\eps} \cdot (\log d) \cdot \sqrt{  n  \cdot \ln \frac{1}{\beta} }  }
    $$
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{theorem: unbiased estimator for  private algorithm}]
    The proof is similar to the one for Theorem~\ref{theorem: unbiased estimator for basic private algorithm}.
    For each user~$u \in [n]$, each~$h \in \IntSet{0}{\log d}$, and each~$\ell \in [d / 2^h]$, define the random variable $z_u[h, \ell]$ as
    $$
        z_u [h, \ell] = 
        \begin{cases}
            (1 + \log d) \cdot \cSvr \cdot \pmbomega{}_u[\ell],\, &\text{if}\, h = h_u, \\
            0,\, &\text{if}\, h \neq h_u. 
        \end{cases}
    $$
    Note that~$\EstPartialsum{ \dyadicInterval{h}{\ell} }$ can be written as $\sum_{u \in [n] } z_u [h, \ell]$.
    We claim that 
    \begin{equation} \label{equa: expectation of z in server}
        \E{ z_u [h , \ell] } = \partialsum{u}{ \dyadicInterval{ h_u }{ \ell } }. 
    \end{equation}
    Via linearity of expectation, we get
    \begin{align*}
        \E{ \EstPartialsum{ \dyadicInterval{h}{\ell} } } 
            = \sum_{u \in [n] } \E{ z_u [h, \ell] } 
            = \sum_{u \in [n] } \partialsum{u}{\dyadicInterval{h}{\ell} } 
            = \partialsum{ \dyadicInterval{h}{\ell} }.
    \end{align*}
    Therefore, for each~$t \in [d]$, 
    \begin{equation*}
        \E{ \EstPorpulationSum{t} } 
        = \sum_{ \dyadicInterval \in \dyadicDecomposition{t} } \E{ \EstPartialsum{ \dyadicInterval } } 
        = \sum_{ \dyadicInterval \in \dyadicDecomposition{t} } \partialsum{ \dyadicInterval } 
        = \PorpulationSum{t}.
    \end{equation*}
    It is left to verify Equation~(\ref{equa: expectation of z in server}).
    If $h_u \neq h$, which happens with probability $1 - 1 / \paren{1 + \log d}$, then $z_u [h, \ell] = 0$; otherwise, conditioning on $h_u = h$, 
    there are two possible cases.
    First, for each $\ell \notin \supp{ h_u }$, $\partialsum{u}{\dyadicInterval{h}{\ell} } = 0$ and it holds that $\E{ z [h, \ell] \mid h_i = h } = 0$.
    Second, consider the $\ell \in \supp{ h_u }$. 
    Assume the indexes in $\supp{ h_u }$ are
    $\ell_1 < \ell_2 < \ldots < \ell_{ \card{ \supp{h_u} } }$.
    For each~$j \in \card{ \supp{h_u} }$, it holds that 
    \begin{align*}
        \E{ z_i [h, \ell] \mid h_i = h }
        &= \E{ (1 + \log d) \cdot \cSvr \cdot W_u [j] \cdot \partialsum{u}{\dyadicInterval{h}{\ell} }  } \\ 
        &= (1 + \log d) \cdot \cSvr \cdot \E{ W_u [j] \cdot \partialsum{u}{\dyadicInterval{h}{\ell} }  }.
    \end{align*}
    Observe that $\E{ W_u [j] \cdot \partialsum{u}{\dyadicInterval{h}{\ell} } }$ equals
    \begin{align*} 
        &\paren{ \partialsum{u}{\dyadicInterval{h}{\ell} } \cdot \P{ W_u [j] = 1 } + (- \partialsum{u}{\dyadicInterval{h}{\ell} } ) \cdot \P{ W_u [j] = - 1 } } \\
        &= \paren{ \P{ W_u [j] = 1} - \P{ W_u [j] = -1 } } \cdot \partialsum{u}{\dyadicInterval{h}{\ell} } \\
        &= 1 / \paren{ \cSvr }  \partialsum{u}{\dyadicInterval{h}{\ell} }. 
    \end{align*}
    It concludes that 
    \begin{align*}
        \E{ z_i [h , r] } 
        &= \E{ z_i [h, \ell] \mid h_i \neq h} \cdot \P{ h_i \neq h } \\
        &\, + \E{ z_i [h, \ell] \mid h_i = h } \cdot \P{ h_i = h } \\
        &= \partialsum{u}{\dyadicInterval{h}{\ell} }.
    \end{align*}
    
\end{proof}




\begin{proof}[Proof of Theorem~\ref{theorem: error of single estimator for private algorithm}]
    For each user~$u \in [n]$, each~$h \in \IntSet{0}{\log d}$, and each~$\ell \in [d / 2^h]$, define the random variable $z_u[h, \ell]$ as in the proof of Theorem~\ref{theorem: unbiased estimator for  private algorithm}.
    Now
    $$
        \begin{aligned}
            \EstPorpulationSum{t} 
                &= \sum_{ \dyadicInterval{h}{\ell} \in \dyadicDecomposition{t} } \EstPartialsum{ \dyadicInterval{h}{\ell} } 
                = \sum_{ \dyadicInterval{h}{\ell}  \in \dyadicDecomposition{t} } \sum_{u \in [n] } z_u [h, \ell] \\
                &= \sum_{u \in [n] } \paren{ \sum_{ \dyadicInterval{h}{\ell}  \in \dyadicDecomposition{t} }  z_u [h, \ell] }.
        \end{aligned}
    $$
    
    \noindent For each $u \in [n]$, define $Y_u = \sum_{ \dyadicInterval{h}{\ell} \in \dyadicDecomposition{t} }  z_u [h, \ell]$. 
    Clearly the $Y_u$ are independent. 
    We will show that $Y_u \in (1 + \log d) \cdot \cSvr \cdot [-1, 1]$.
    Applying Corollary~\ref{corollary: confident interval of hoeffding}, we see that with probability at most $\beta$, 
    $$
        \card{ \EstPorpulationSum{t} - \E{ \EstPorpulationSum{t} } }
        = |Y - \E{ Y } | \ge (1 + \log d) \cdot \cSvr \cdot \sqrt{ 2 n \cdot \ln \frac{2}{\beta} }.
    $$
    Recall that $\cSvr \le 2 \cdot \paren{ e^{ \tildeeps} + 1} / \paren{ e^{ \tildeeps } - 1 }$.
    Further, when $\tildeeps < 1$, $e^{\tildeeps} + 1\in O(1)$ and 
    $$
        e^{\tildeeps} - 1 \in \Theta ( \tildeeps )
            = \Theta \paren{ \frac{\eps}{6 \sqrt{k \ln \paren{ 12 (k + 1) \sqrt{ 1 + \ln (1 / \eps) } / \eps }  } } }.
    $$
    Combining with that $\E{ \EstPorpulationSum{t} } = \PorpulationSum{t}$, it holds that with probability at least $1 - \beta$,
    $$
        \big| \EstPorpulationSum{t} - \PorpulationSum{t} \big| \in O \paren{ \frac{ \sqrt{k \cdot \paren{ \ln k + \ln (1 / \eps) } } } {\eps} \cdot (\log d) \cdot \sqrt{  n  \cdot \ln \frac{1}{\beta} }  }.
    $$
    
    It is left to prove that $Y_u \in (1 + \log d) \cdot \cSvr \cdot [-1, 1]$.
    By Fact~\ref{observation: nodes be in different level}, dyadic intervals in $\dyadicDecomposition{t}$ have distinct orders. 
    The definition of~$z_u$ guarantees that for all $\dyadicInterval{h}{\ell}  \in \dyadicDecomposition{t}$, there is at most non-zero $z_u[h, \ell]$, which has value either $-(1 + \log d) \cdot \cSvr$ or $(1 + \log d) \cdot \cSvr$.
    
\end{proof}













==> lower-bound.tex <==
\section{Lower Bound} \label{sec:lower bound}


In the section, we prove a lower bound for the problem.

\begin{theorem} \label{theorem: lower bound of the problem}
    Assuming that $\eps \le 1$, and $\sqrt{n} \ge ( 1 / \eps ) \cdot \sqrt{k \cdot \log ( d / k ) }$, 
    for every~$\eps$-locally differentially private~$(\alpha, \beta)$-accurate protocol, if~$\beta > 1 / 2$, 
    then 
    $$
        \alpha \in  \Omega  \paren{ \frac{ 1 } {\eps} \cdot \sqrt{  k \cdot n  \cdot \ln \frac{d}{\beta} }  }.
    $$
\end{theorem}


\subsection{Minimax Framework}

We consider the set  $\cD \doteq \set{ x \in \set{ -1, 0, 1 }^d : \norm{ x }_0 \le k }$, where $\norm{ \cdot }_0$ is the number of non-zero dimensions in $x$.
With standard computation, we have the following lemma, the proof of which we include in the appendix,

\begin{lemma} \label{lemma: size of D}
    $\log |\cD| \in \Theta \paren{ k \log \frac{d}{k} }$.
\end{lemma}

Let $\simplex(\cD)$ be the collection of all possible distributions over $\cD$, and $\theta : \simplex (\cD ) \rightarrow [-n, n]^d$ be defined by
\begin{align}
    \theta( P ) \doteq n \cdot \sum_{ x \in \cD } x \cdot P ( x ),\quad   \forall P \in \simplex ( \cD),\,
\end{align}
where $P (x )$ is the probability of $x$ specified by $P$.
$\theta$ is a linear mapping between $\simplex (D)$ and~$[-n, n]^d$:
for each $P, P' \in \simplex(D)$, $\eta \in [0, 1]$, let $\paren{\eta P + (1 - \eta) P'}$ be the distribution defined by~$\big(\eta P + (1 - \eta) P' \big) (x) \doteq \eta \cdot P(x) + (1 - \eta) \cdot P'(x), \forall x \in \cD$; then 
\begin{fact}
    $
        \theta\big(\eta P + (1 - \eta) P' \big) = \eta \cdot \theta(P) + (1 - \eta) \cdot \theta( P' ). 
    $
\end{fact}


Given a fixed distribution $P$, the users' data, denoted by $X = \paren{ X_1, \ldots, X_n } \in \cD^n$, are assumed to be drawn from $P$ identically and independently at random.
Let $\algoClientSeq{} = \set{ \algoClient{}^{ (u) } }$ be a sequence of randomized algorithms, such that $\algoClient{}^{ (u) } : \set{ -1, 0, 1 }^d$ $\rightarrow \cY, u \in [n]$ are $(\eps, \delta)$-differential private.
Each data $X_u$ is obscured by $\algoClient{}^{ (u) }$ independently, whose output $Y_u = \algoClient{}^{ (u) } ( X_u ) \in \cY$ is then reported to the server.
Based on the reports $Y = \algoClientSeq{} (X) = (Y_1, \ldots, Y_n)$, of interest are two kinds of estimation task.

\noindent \textit{Sample Sum.} The server invokes an algorithm $\hat f: \cY^n \rightarrow [-n, n]^d$, algorithm that outputs a vector $\hat f (Y) \in [-n, n]^d$, as the estimate of sampled sum $f (X) \doteq \sum_{ u \in [n] } X_u$.
Note that 
$
    \E{ f } = \sum_{u \in [n] } \E{ X_u } = n \cdot \sum_{x \in \cD } x \cdot P( x ) = \theta (P).
$
The solution quality of $\hat f$ is measured by the smallest $\ell_\infty$-norm of $\hat f - f$ (with constant probability), denoted by
$$
    \mfrkM ( \hat f, P, \algoClientSeq{} ) \doteq \inf \set{ \alpha :  \P{ \norm{ \hat f - f  }_\infty \le \alpha } > 3 / 4 }.
$$


\noindent \textit{Expected Sum.} The server invokes an algorithm $\hat \theta: \cY^n \rightarrow [-n, n]^d$, that outputs a vector $\hat \theta (Y_1, \ldots, Y_n) \in [-n, n]^d$, as the estimate of expected sum $\theta( P )$.
The solution quality of $\hat \theta$ is measured by the expected $\ell_\infty$-norm of $\hat \theta - \theta$, denoted by
$$
   \mfrkM ( \hat \theta, P, \algoClientSeq{} ) \doteq \inf \set{ \alpha : \P{ \norm{ \hat \theta - \theta  }_\infty \le \alpha } \ge 1 / 2  }.
$$

\begin{definition}
    For a (fixed) sequence of client-side algorithms $\algoClientSeq{} = \set{ \algoClient{}^{ (u) } }$, define the minimax errors by
    \begin{align*}
        \mfrkM ( f, \algoClientSeq{} ) \doteq \min_{ \hat f } \max_{ P } \mfrkM ( \hat f, P, \algoClientSeq{} ) \\
        \mfrkM ( \theta, \algoClientSeq{} ) \doteq \min_{ \hat \theta } \max_{ P }\mfrkM ( \hat \theta, P, \algoClientSeq{} )
    \end{align*}
    where the maximum is over all possible distributions defined on $\cD$, and the minimum is over all possible functions $\hat f: \cY^n \rightarrow [-n, n]^d$ ($\hat \theta: \cY^n \rightarrow [-n, n]^d$).
\end{definition}

The main result of this section is stated as follows:

\begin{lemma} \label{lemma: lower bound on f minimax error}
    For all $\eps \in O(1)$ and $\delta \in o( \frac{ \eps }{ n \log n} )$, and all possible sequences of algorithms $\algoClientSeq{} = \set{ \algoClient{}^{ (u) } }$, such that $\algoClient{}^{ (u) }, : u \in [n]$ are $(\eps, \delta)$-differential private,
    $$
        \mfrkM ( f, \algoClientSeq{} )  \in \Omega \paren{ \frac{1}{ \eps } \sqrt{ n \cdot k \cdot \log \frac{d}{k} } }.
    $$
\end{lemma}

The proof of the lemma is based on a reduction from the lower bound of $\mfrkM ( \theta, \algoClientSeq{} )$, which we will prove in the next section, and relies on an upper bound of $\E{ \norm{ f - \theta  }_\infty } \le \sqrt{n \cdot k}$, the proof of which we defer to the end of the section.


\begin{lemma} \label{lemma: lower bound on theta minimax error}
    Let $\eps \in O(1)$ and $\delta \in o( \frac{ \eps }{ n \log n} )$, and assume that $\sqrt{n} \ge ( 1 / \eps ) \cdot \sqrt{k \cdot \log ( d / k ) }$.
    For all possible sequences of algorithms $\algoClientSeq{} = \set{ \algoClient{}^{ (u) } }$, such that $\algoClient{}^{ (u) }, u \in [n]$ are $(\eps, \delta)$-differential private,
    $$
        \mfrkM ( \theta, \algoClientSeq{} ) \in \Omega \paren{ \frac{1}{ \eps } \sqrt{ n \cdot k \cdot \log \frac{d}{k} } }.
    $$
\end{lemma}

\begin{lemma}
    \label{lemma: upper bound on sample sum deviation}
    For all $P \in \simplex(\cD )$, it holds that
    \begin{align} \label{ineq: upper bound on sample sum deviation}
        \E{\norm{ f - \theta  }_\infty } \le \sqrt{n \cdot k}.
    \end{align}
\end{lemma}


\begin{proof}[\textbf{Proof of Lemma~\ref{lemma: lower bound on f minimax error}}]

    Suppose that the lemma does not hold, 
    then there is a sequence client side algorithms $\algoClientSeq{}$ and a server side algorithm  $\hat f{}$, such that for all $P \in \simplex ( \cD )$, we have
    \begin{align*} 
       \mfrkM ( \hat f, P, \algoClientSeq{} ) \in o \paren{ ( 1 / \eps ) \cdot \sqrt{ n \cdot k \cdot \log ( d / k ) } },
    \end{align*}
    which implies that 
    \begin{equation} \label{ineq: false assumption of error}
        \P{ \norm{ \hat f - f  }_\infty \in o \paren{ ( 1 / \eps ) \cdot \sqrt{ n \cdot k \cdot \log ( d / k ) } } } > 3 / 4.
    \end{equation}
    Via Inequality~(\ref{ineq: upper bound on sample sum deviation}) and Markov's inequality, we get 
    \begin{equation} \label{ineq: prob upper bound on sample sum deviation}
        \P{ \norm{ f - \theta  }_\infty \ge 4 \cdot \sqrt{n \cdot k } } \le 1 / 4. 
    \end{equation}
    Via triangle inequality, it holds that for each $P \in \simplex ( \cD )$,
    \begin{equation} \label{ineq: error decomp of hat f - theta}
        \norm{ \hat f - \theta  }_\infty 
        \le
        \norm{ \hat f - f  }_\infty 
        +
        \norm{ f - \theta  }_\infty .
    \end{equation}
    

    Combining inequalities~(\ref{ineq: false assumption of error}),~(\ref{ineq: error decomp of hat f - theta}) and~(\ref{ineq: prob upper bound on sample sum deviation}), we conclude that there is a sequence client side algorithms $\algoClientSeq{}$ and a server side algorithm $\hat f{}$, such that for all $P \in \simplex ( \cD )$,
    $$
        \P{ \norm{ \hat f - \theta  }_\infty \in o \paren{ ( 1 / \eps ) \cdot \sqrt{ n \cdot k \cdot \log ( d / k ) } } } \ge 1 / 2,
    $$
    which is a contradiction to Lemma~\ref{lemma: lower bound on theta minimax error}.
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lemma: upper bound on sample sum deviation}]
    Recall that $f = \sum_{u \in [n] } X_u$, where $X_u \sim P$ for each $u \in [n]$, and that $\theta( P ) \doteq n \cdot \sum_{ x \in \cD } x \cdot P ( x )$.
    Hence,
    $$
        \E{ f }
        = \sum_{u \in [n] } \E{ X_u }
        = n \cdot \sum_{ x \in \cD } x \cdot P ( x )
        = \theta( P ).
    $$
    Since~$\E{ \norm{ f - \theta }_\infty } \le \E{ \norm{ f - \theta }_2 }$, we prove the lemma if we can bound~$\E{ \norm{ f - \theta }_2 }$ by $\sqrt{n \cdot k }$.
    Since $f$ is an $d$-dimensional vector, for each $t \in [d]$, denotes its $t^{(th)}$ coordinate by $f[t]$. 
    Similarly, denote the $t^{(th)}$ coordinates of $\theta(P)$ and $X_u, u \in [n]$ by $\paren{ \theta(P) }[t]$ and $X_u[t]$, respectively. 
    
    Via the Jensen's inequality
    \begin{align*}
        \E{ \norm{ f - \theta }_2 }
        &\le \sqrt{  \sum_{t \in [d] } \E{ \paren{ f [t] - \paren{ \theta(P) } [t] }^2 } }
    \end{align*}
    For each $t \in [d]$, $f[t] = \sum_{u \in [n] } X_u [t]$ is a sum of $n$ independent random variables, we have
    \begin{align*}
        \E{ \paren{ f[t] -  \paren{ \theta(P) } [t] }^2 }
         & = \Var{ f[t] }
        = \sum_{u \in [n] } \Var{ X_u [t] }.
    \end{align*}
    As $X_u [t] \in \set{-1, 0, 1}$,
    $
        \Var{ X_u [t] } \le \E{ \paren{ X_u [t]  }^2 } = \P{ X_u [t] \neq 0 }
    $.
    It follows that
    \begin{align*}
        \E{ \norm{ f - \theta }_2 }
         & \le \sqrt{  \sum_{u \in [n] } \sum_{t \in [d] } \P { X_u [t] \neq 0 } }
    \end{align*}
    Since $X_u$ is sampled from $\cD$, it contains at most $k$ non-zero dimensions and
    \begin{align*}
        &\sum_{t \in [d] } \P { X_u [t] \neq 0 }
        = \sum_{t \in [d] } \sum_{ x \in \cD } \dsone{} \big[ x [ t ] \neq 0 \big] \cdot P( x ) \\
        & = \sum_{ x \in \cD } \paren{ \sum_{t \in [d] } \dsone{} \big[ x [ t ] \neq 0 \big] } \cdot P( x ) 
        \le \sum_{ x \in \cD } k \cdot P( x )
        = k.
    \end{align*}
    It concludes that $\E{ \norm{ f - \theta }_\infty } \le \sqrt{ n \cdot k}$.
\end{proof}


\subsection{Proof of Lemma~\ref{lemma: lower bound on theta minimax error}}

\begin{definition}[$\eta$-degrading Channel \cite{BS15}] Given $\eta \in [0, 1]$, a $\eta$-degrading channel $W^{ (\eta) }: \cD \rightarrow \cD$ is a randomized mapping defined by follows:
    $$
        W^{ (\eta) } ( x ) =
        \begin{cases}
            x, & \text{w.p.}\, \eta,     \\
            V,       & \text{w.p.}\, 1 - \eta.
        \end{cases}
    $$
    where $V$ is a uniform random variable over $\cD$.
\end{definition}

For each $u \in [n]$, denote $\algoClient{}^{ (u) } \circ W^{ (\eta) } : \cD \rightarrow \cY$ the composition of $\algoClient{}^{ (u) }$ and $W^{ (\eta) }$, such that for each $x \in \cD$,
$
    \algoClient{}^{ (u) } \circ W^{ (\eta) } ( x ) = \algoClient{}^{ (u) } \paren{ W^{ (\eta) } ( x ) }.
$
Denote $\algoClientSeq{} \circ W^{ (\eta) } \doteq $ $\set{ \algoClient{}^{ (u) } \circ W^{ (\eta) } }$, where each $\algoClient{}^{ (u) }, u \in [n]$ is composed with an independent copy of $W^{ (\eta) }$.

\begin{fact}[\cite{BS15}]
    The composition $\algoClient{}^{ (u) } \circ W^{ (\eta) }$ of an $\eta$-degrading channel $W^{ (\eta) }$ with an $(\eps, \delta)$-locally differentially private algorithm $\algoClient{}^{ (u) }$ yields a $( O( \eta \eps), O( \eta \delta) )$-locally differentially private algorithm.
\end{fact}

In what follows, we write the probability~$\P{ \norm{ \hat \theta - \theta  }_\infty \le \alpha }$ explicitly as
$$
    \P{X \sim P, Y \sim \algoClientSeq{} (X) }{ \norm{ \hat \theta - \theta  }_\infty \le \alpha } \,
    \quad \text{or}\, 
    \P{ P , \algoClientSeq{} }{ \norm{ \hat \theta - \theta  }_\infty \le \alpha },
$$
when $X = \paren{ X_1, \ldots, X_n } \in \cD^n$ are sampled from the distribution $P$ and $Y = (Y_1, \ldots, Y_n)$ are the outputs of $\algoClient{}^{ (u) } (X_u), u \in [n]$.
We are interested in the following errors. 
\begin{align*}
    \mfrkM ( \hat \theta, P, \algoClientSeq{} ) 
        &= \inf \set{ \alpha : \P{P, \algoClientSeq{} }{ \norm{ \hat \theta - \theta  }_\infty \le \alpha } \ge \frac{1}{2}  }, \\
    \mfrkM ( \hat \theta, P, \algoClientSeq{} \circ W^{ (\eta) } ) 
        &= \inf \set{ \alpha : \P{P, \algoClientSeq{} \circ W^{ (\eta) } }{ \norm{ \hat \theta - \theta  }_\infty \le \alpha } \ge \frac{1}{2}  }.
\end{align*}


\begin{lemma}
    For every sequence of client-side algorithms $\algoClientSeq{} = \set{ \algoClient{}^{ (u) } }$, if
    \begin{align*}
        \min_{ \hat \theta } \max_{ P \in \simplex ( \cD ) } \mfrkM ( \hat \theta, P, \algoClientSeq{} ) 
        < \frac{ \eta \cdot n}{ 10 },
    \end{align*}
    then
    \begin{align*}
        \min_{ \tilde \theta } \max_{ P \in \simplex ( \cD ) } \mfrkM ( \tilde \theta, P, \algoClientSeq{} \circ W^{ (\eta) } ) 
        < \frac{ n }{ 10 }.
    \end{align*}

\end{lemma}

\begin{proof}
    Suppose there exits an algorithm $\hat \theta: \cY^n \rightarrow [-n, n]^d$ such that
    \begin{equation}
        \max_{ P \in \simplex ( \cD ) } \mfrkM ( \hat \theta, P, \algoClientSeq{} ) 
        < \frac{ \eta \cdot n }{ 10 },
    \end{equation}
    Define the algorithm $\tilde \theta: \cY^n \rightarrow [-n, n]^d$ by
    $$
        \tilde \theta (y_1, \ldots, y_n) = \frac{1}{ \eta } \paren{ \hat \theta (y_1, \ldots, y_n) - ( 1 - \eta) \cdot \theta ( U ) }.
    $$
    where $U$ denotes the uniform distribution over $\cD$.
    We will prove
    $$
        \max_{ P \in \simplex ( \cD ) } \mfrkM ( \tilde \theta, P, \algoClientSeq{} \circ W^{ (\eta) } ) 
        < \frac{n}{10}.
    $$
    For each $P \in \simplex ( \cD )$,
    \begin{align*}
        \tilde \theta (y_1, \ldots, y_n) - \theta (P)
         & = \frac{1}{ \eta } \paren{ \hat \theta (y_1, \ldots, y_n) - ( 1 - \eta) \cdot \theta ( U ) } - \theta (P) \\
         & = \frac{1}{ \eta } \paren{ \hat \theta (y_1, \ldots, y_n) -  \theta \paren{ P^{ (\eta) } } },
    \end{align*}
    where $P^{ (\eta) } = ( 1 - \eta) \cdot  U  + \eta \cdot  P$.
    Further, suppose that $X_u \sim P$, $u \in [n]$ are independent random variables, then
    $
        X_u^{ (\eta) } \doteq W^{ (\eta) } (X_u) \sim P^{ (\eta) }, u \in [n].
    $
    Let $Y_u = Y_u^{ (\eta) } = \algoClient{}^{ (u) } \paren{ W^{ (\eta) } (X_u) }$, $u \in [n]$.
    Then by assumption, we have 
    $$
        \P{ P^{ (\eta) }, \algoClientSeq{} } { \norm{ \hat \theta - \theta  }_\infty \le \frac{\eta n}{10} } \ge \frac{1}{2} 
    $$
    But when~$\hat \theta (y_1, \ldots, y_n) -  \theta \paren{ P^{ (\eta) } } \le \eta n / 10$, we have 
    $
        \tilde \theta (y_1, \ldots, y_n) - \theta (P) \le n / 10.
    $
    Therefore, 
    $$
        \P{ P, \algoClientSeq{} \circ W^{ (\eta) } } { \norm{ \hat \theta - \theta  }_\infty \le \frac{ n}{10} } \ge \frac{1}{2} 
    $$
\end{proof}

\begin{lemma}
    For each sequence of client-side algorithms $\algoClientSeq{} = \set{ \algoClient{}^{ (u) }  }$, we have
    \begin{align*}
        \min_{ \tilde \theta } \max_{ P \in \simplex ( \cD ) } \mfrkM ( \tilde \theta, P, \algoClientSeq{} \circ W^{ (\eta) } ) 
        \ge \frac{ n }{ 2 }.
    \end{align*}
\end{lemma}

\begin{proof}
    Suppose there is an $\tilde \theta : \cY^n \rightarrow [-n, n]^d$, s.t., 
    $$
        \max_{ P \in \simplex ( \cD ) } \mfrkM ( \tilde \theta, P, \algoClientSeq{} \circ W^{ (\eta) } ) 
        < \frac{ n }{ 2 }. 
    $$
    It follows that, 
    \begin{equation}
        \label{ineq: lower probability bound of infty error}
         \forall P \in \simplex ( \cD ),\,
         \P{P, \algoClientSeq{} \circ W^{ (\eta) } }{ \norm{ \hat \theta - \theta  }_\infty < \frac{ n }{ 2 } } \ge \frac{4}{5}. 
    \end{equation}
    Let $\cP \doteq \set{ P_{ x } : x \in \cD } \subset \simplex ( \cD )$ be the collection of point-supported distributions, such that $\forall x \in \cD$, $P_{ x }$ assigns $x$ probability $1$ and all other points $0$.
    Therefore, $\theta ( P_{ x } ) = n \cdot x$.
    We will prove that 
    \begin{equation} 
        \label{ineq: average lower prob}
         \sum_{ P_x \in \cP } \frac{1}{ | \cP | }  \P{ P_x, \algoClientSeq{} \circ W^{ (\eta) } }{ \norm{ \hat \theta - \theta  }_\infty \ge \frac{ n }{ 2 } } 
         \ge \frac{1}{2}.
    \end{equation}
    This implies a contradiction to Equation~(~\ref{ineq: lower probability bound of infty error}):
    $$
        \exists P \in \cP,\,
        \P{ P_x, \algoClientSeq{} \circ W^{ (\eta) } }{ \norm{ \hat \theta - \theta  }_\infty \ge \frac{ n }{ 2 } } \ge \frac{1}{2}.
    $$ 
    {\it Proof of Inequality~(\ref{ineq: average lower prob}):}
    Let $V \sim U$ be a uniform random variable over $\cD$.
    Then it suffices to verify that 
    $$
        \E{V }{ \P{ P_V, \algoClientSeq{} \circ W^{ (\eta) } }{ \norm{ \hat \theta - \theta  }_\infty \ge \frac{ n }{ 2 } }  }
        \ge 
        \frac{1}{2}. 
    $$
    The error~$\norm{ \tilde \theta - \theta  }_\infty$ can be interpreted as follows:
    first, $V$ is drawn uniformly from $\cD$; then, each $X_u$ is sampled independently according to $P_{ V }$.
    Via definition of $P_{ V }$, we have $X_u = V$;
    each $X_u$ is further processed independently by $\algoClient{}^{ (u) } \circ W^{ (\eta) }$, to compute an obscured version $Y_u = \algoClient{}^{ (u) }( W^{ (\eta) } ( X_u) ) = \algoClient{}^{ (u) }( W^{ (\eta) } ( V ) )$;
    finally, based on $Y = (Y_1, \ldots, Y_n)$, $\tilde \theta(Y_1, \ldots, Y_n)$ computes an estimate of $\theta (P_V) = n \cdot V$.
    $\norm{ \tilde \theta - \theta  }_\infty$ measures the deviation of~$\tilde \theta(Y_1, \ldots, Y_n)$ from~$n \cdot V$.
    Now, define the function $\psi: \cY^n \rightarrow \cD$ by
    $$
        \psi(y_1, \ldots, y_n) 
        = 
        \argmin_{ x \in \cD } \norm{ n \cdot x - \tilde \theta (y_1, \ldots, y_n) }_\infty
    $$
    \begin{claim} 
        \label{claim: lower bound of wrong guess}
        $
            \P { \psi (Y_1, \ldots, Y_n) \neq V  }
            \ge 
            \frac{1}{2}.
        $
    \end{claim}
    \noindent We defer the proof of the claim to the end of the section. 
    Based on the claim, it suffices to show that 
    \begin{equation}
        \label{ineq: estimation to decision}
        \E{V }{ \P{ P_V, \algoClientSeq{} \circ W^{ (\eta) } }{ \norm{ \hat \theta - \theta  }_\infty \ge \frac{ n }{ 2 } }  }
        \ge 
        \P { \psi (Y_1, \ldots, Y_n) \neq V  }.
    \end{equation}
    \noindent For each~$x \in \cD$, consider the $\ell_\infty$ ball centered at~$n \cdot x$ defined by
    $$
        \cB(n \cdot x) \doteq \set{ \tilde{x} \in [-n, n]^d : \norm{ n \cdot x - n \cdot \tilde{x} }_\infty < n / 2}.
    $$ 
    For each $x, x' \in \cD$, if $x \neq x'$, then they differ in at least one dimension.
    Therefore, the balls $\cB(n \cdot x), x \in \cD$ are disjoint. 
    Therefore, if~$\tilde \theta (y_1, \ldots, y_n) \in \cB(n \cdot x)$ for some $x \in \cD$, then we must have that~$\psi(y_1, \ldots, y_n) = x$. 
    Conditioned on $V = x$, 
    \begin{equation*}
        \P{ P_x, \algoClientSeq{} \circ W^{ (\eta) } } { \norm{ \tilde \theta - n \cdot x  }_\infty < \frac{n}{2} }
        \le
        \P{ P_x, \algoClientSeq{} \circ W^{ (\eta) } } { \psi (Y_1, \ldots, Y_n) = x },
    \end{equation*}
    or equivalently,
    $$
        \P{ P_x, \algoClientSeq{} \circ W^{ (\eta) } } { \norm{ \tilde \theta - n \cdot x }_\infty \ge \frac{n}{2} }
        \ge
        \P{ P_x, \algoClientSeq{} \circ W^{ (\eta) } } { \psi (Y_1, \ldots, Y_n) \neq x  }.
    $$
    Taking expectation over all $x \in \cD$, and applying that $\theta(P_V) = n \cdot V$ finishes the proof for Inequality~(\ref{ineq: estimation to decision}).

\end{proof}

To prove Claim~\ref{claim: lower bound of wrong guess}, we rely on the following facts. 


\begin{fact}[Fano's Inequality \citep{duchi2021information}] Let $V$ be uniform on $\cD$. For the Markov chain $V \rightarrow (Y_1, \ldots, Y_n) \rightarrow \psi(Y_1, \ldots, Y_n)$, it holds that
    $$
        \P{ \psi (Y_1, \ldots, Y_n) \neq V } \ge { 1 - \frac{ I( Y_1, \ldots Y_n; V ) + \log 2 }{ \log | \cD |} }
    $$
\end{fact}

\begin{fact}[\cite{BS15}]
    Let $V$ be uniformly distributed over $\cD$. Let $\algoClient{}: \cD \rightarrow \cY$ be $(\eps, \delta)$-differentially private, and let $Y = \algoClient{} ( V )$. Then, we have that
    $$
        I( Y ; V ) = O \paren{ \eps^2 + \frac{ \delta }{ \eps } \log ( | \cD | ) + \frac{ \delta }{ \eps } \log \frac{\eps }{ \delta } }.
    $$
\end{fact}

\begin{fact}[\citep{duchi2021information}]
    Suppose that~$Y_1, \dots, Y_n$ are conditional independent given $V$, then
    \begin{align*}
        I(Y_1, \ldots, Y_n ; V)
        \le \sum_{u \in [n] } I(Y_u ; V).
    \end{align*}
    
\end{fact}

\begin{proof}[Proof of Claim~\ref{claim: lower bound of wrong guess}]
    Since $\algoClient{}^{ (u) } \circ W^{ (\eta) }$ is $( O(\eta \eps), O( \eta \delta) )$ differentially private, if $Y_u = \algoClient{}^{ (u) } \paren{ W^{ (\eta) } ( V ) }$, we have
    $$
        I(Y_u ; V) = O \paren{ \eta^2 \eps^2 + \frac{ \delta }{ \eps } \log ( | \cD | ) + \frac{ \delta }{ \eps } \log \frac{\eps }{ \delta } }.
    $$  
    Hence, $I(Y_1, \ldots, V_n ; V) \in O \paren{ n \cdot \eta^2 \eps^2 + n \cdot \frac{ \delta }{ \eps } \log ( | \cD | ) + n \cdot \frac{ \delta }{ \eps } \log \frac{\eps }{ \delta } }$.
    Using that $\delta \in o( \eps / (n \cdot \log n)$, and setting $\eta = C_\eta \cdot \paren{ \sqrt{ \frac{ \log | \cD | }{n \eps^2}} }$, we get
    $$
        O \paren{ n \cdot \eta^2 \eps^2 + n  \frac{ \delta }{ \eps } \log ( | \cD | ) + n \frac{ \delta }{ \eps } \log \frac{\eps }{ \delta } }
        \in
        O \paren{ C_\eta^2 \log |\cD| + \frac{ \log |\cD| }{\log n} }.
    $$
    Hence, 
    \begin{align*}
        \P{ \psi (Y_1, \ldots, Y_n) \neq V } 
            &\ge { 1 - \frac{ I( Y_1, \ldots Y_n; V ) + \log 2 }{ \log | \cD |} } \\
            &\in  1 - \Omega \paren{ C_\eta^2 + \frac{1}{ \log n} + \frac{\log 2}{\log | \cD | } }.
    \end{align*}
    When~$n$ and~$|\cD|$ are large enough, and by picking~$C_\eta$ properly, we have~$\P{ \psi (Y_1, \ldots, Y_n) \neq V } \ge 1 / 2$.

\end{proof}











==> related-work.tex <==
\section{Related Works} \label{sec: review}

Data analysis under {\it continual observation} was studied in the central model of differential privacy~\citep{DworkNPR10, ChanSS11}, where a trusted curator, to which the clients report their true data,  perturbs and releases the aggregated data. 
Given a stream of Boolean values,~$0$ and~$1$, differentially private frequency estimation algorithms were independently proposed by both~\citeauthor{DworkNPR10}~\citep{DworkNPR10} and~\citeauthor{ChanSS11}~\citep{ChanSS11}, which output at each time period an estimate of the number of~$1$s appearing so far. 
These algorithms guarantee an error of~$O \paren{ 1 / \eps \cdot \log^{1.5} t }$ (omitting failure probability) at each time~$t$.

In the local model, the \emph{memoization} technique was proposed and deployed for continual collection of counter data~\citep{EPK14, DKY17}, where noisy answers for all elements in the domain are memorized. 
However, as pointed out by~\citep{DKY17}, this technique can violate differential privacy. 


Our algorithmic framework is inspired by the work of~\citeauthor{EFMRTT19}~\cite{erlingsson2020amplification}, who proposed to exploit the potential sparsity of users' data 
if it changes infrequently.
Here we provide a succinct description of their protocol under the notations and framework of our paper.
The protocol in~\cite{erlingsson2020amplification} requires
an additional sampling step: each user~$u$ samples uniformly and keeps only one non-zero coordinate of~$\UsrDerivative{u}$, and sets all other non-zero coordinates to~$0$.
Therefore, there can be at most one non-zero partial sum with sampled order~$h_u$.
This partial sum is perturbed by the basic randomizer~$\cR$ (Equation~(\ref{equa: def of basic randomizer})) with~$\tildeeps = \eps / 2$, resulting in a~$\paren{ \cGap }^{-1} \in \Omega \paren{ 1 / \eps }$.
However, due to the additional sampling step, the server side estimator of~$\EstPartialsum{ \dyadicInterval{h}{j} }$ (Algorithm~\ref{algo: server}, line~\ref{line: algo: server: update partial sum}) needs to be multiplied by an additional factor of~$k$.
Via similar analysis as Lemma~\ref{lemma: error of single estimator for basic private algorithm},
the error guarantee of their protocol involves a factor of~$k$, instead of~$\sqrt{k}$.

The composed randomizer~$\tilde{\cR}$ presented in this paper builds on the composed randomizer proposed by~\citeauthor{BNS19}~\citep{BNS19}.
Their design
focused on preserving the statistical distance between the distribution of the output of the composed randomizer, and joint distribution of~$k$ independent randomized responses.
This difference in the problem setting prompts the non-trivial changes in parameters, assumptions and analysis.
The \citeauthor{BNS19} proof~\citep{BNS19} relies extensively on concentration and anti-concentration inequalities.
Their design can only achieve
$        
    \cGap \in 
    O \Big( {\eps} / {\sqrt{k \ln ( k / \eps) } } + \big( \frac{ \eps }{ k \ln ( k / \eps) } \big)^{2 / 3} \Big)
$ 
(detailed discussion and proof are in Appendix~\ref{appendix: subsec: bun randomizer}). 
When the first term dominates, this simplifies to~$\cGap \in O ( {\eps} / {\sqrt{k \ln ( k / \eps) } } )$, which implies that~$(\cGap)^{-1} \in \Omega ( {\sqrt{k \ln ( k / \eps) } } / {\eps} )$.
If we apply this composed randomizer to our framework, according to Lemma~\ref{lemma: error of single estimator for basic private algorithm}, this leads to an error that scales at least with~${\sqrt{k \ln ( k / \eps) } } / \eps$.
In comparison, our composed randomizer reduces this to at most~$\sqrt{k} / \eps$. 
Further, \citeauthor{BNS19}'s original design~\citep{BNS19} applies only to offline inputs. 
We overcome this limitation by proposing the pre-computation technique for converting the algorithm to an online one.


Finally, the recent independent parallel work by~\citeauthor{zhou2021locally}~\citep{zhou2021locally}
considers the problem in the offline setting, where there is no requirement for the server to report the estimate at each time step.
They describe a protocol that achieves an error of~$O ( (1 / \eps) \cdot \sqrt{  k \cdot (\log n / \beta) \cdot n  \cdot \log ( d /  \beta ) } )$.
Their client-side algorithm involves hashing the coordinates of user data into a table, and reporting a perturbed version of the hash table to the server. 
Since the value of the entries of the hash table depends on all coordinates of the user data, it is unclear how to convert this algorithm into an online one. 


